Probabilistic Modelling is Sufficient for Causal Inference

Causal inference is a key research area in machine learning, yet confusion reigns over the tools needed to tackle it. There are prevalent claims in the machine learning literature that you need a bespoke causal framework or notation to answer causal questions. In this paper, we want to make it clear that you \emph{can} answer any causal inference question within the realm of probabilistic modelling and inference, without causal-specific tools or notation. Through concrete examples, we demonstrate how causal questions can be tackled by writing down the probability of everything. Lastly, we reinterpret causal tools as emerging from standard probabilistic modelling and inference, elucidating their necessity and utility.

==> 2-intervention-example.tex <==
\examplebox{Interventions on Aspirin Dose}{
    \examplesec{Inference question}
    In the observed world, in which the subjects decide their own aspirin dosage, we've surveyed people to collect a dataset $\mathcal{D}=\{(z_i, t_i, y_i)\}_{i=1}^N$. We want to use this dataset to answer the question: what is the expected effect of intervening to assign someone a given dose of aspirin $T$ on their headache duration $Y$ on average? By how much would doubling someone's assigned aspirin dose reduce their headache duration?

    \examplesec{Model and assumptions}
    Let's begin by setting up a model in which the two settings of interest --- the observed and the interventional --- are modelled explicitly. In addition to the random variables corresponding to the observed dataset $\{(Z_i, T_i, Y_i)\}_{i=1}^N$, which we assume has been generated as described in eq.~\ref{aspirin-observed-model-eqs} in the previous section, we also define variables $Z^*$, $T^*$, $Y^*$, which correspond to the intervened-upon setting. We can then make assumptions about how these two settings are related and consequently write down a joint distribution over those.
    
    % summary: dependence of dose on Z in interventional 
    Let's first consider the dependence of $T^*$ on $Z^*$ in the intervened-upon world. We're interested in a hypothetical intervention where we \emph{assign} people a higher dose. To isolate the effect of aspirin, we are interested in assignment of a given dose regardless of the subject's initial headache severity. Hence, the dose $T^*$ in the interventional setting ought to be independent of the headache severity $Z^*$. To represent the belief that we are manipulating the system to assign a specific dose $t^*$ independently of $Z^*$, we can specify:
    \begin{align}
        T^*=t^* && \Longleftrightarrow && p(T^*=t)=\delta (t^* - t)
    \end{align}
    where $\delta(\cdot)$ is a Dirac delta function. Setting $T^*$ to be delta distributed means that:
    \begin{equation}
        p(\cdot)=\int p(\cdot, T^*\teq~t)~dt=\int p(\cdot|T^*\teq~t)\underbrace{p(T^*\teq~t)}_{\delta (t^* - t)}dt= p(\cdot~|T^*\teq~t^*)\label{eq:intervention-marginal-is-cond}
    \end{equation}
    This identity that will come in useful below.

    %Note that this corresponds to an experimental setting
    In this hypothetical interventional setting, we believe that the physical mechanism determining the headache duration $Y^*$ based on the initial headache severity $Z^*$ and aspirin dose ingested $T^*$ remains unchanged. Hence, in the intervened-upon world, we assume that conditional distribution of headache duration $Y^*$ conditioned on $T^*$ and $Z^*$ --- $p_{\boldsymbol{\theta}} (Y^*\tighteq~y^*|T^{*}\tighteq~t^*,Z^*\tighteq~z^*)$ --- remains the same as in the observed world --- $p_{\boldsymbol{\theta}}~(Y_i\tighteq~y|T_i\tighteq~t, Z_i\tighteq~z)$. For notational convenience, we'll write $q(\cdot)$ in place of $p(\cdot)$ when referring to distribution functions over interventional variables $Z^*, T^*, Y^*$ when using the machine learning short-hand. For instance, we'll write $q_{\boldsymbol{\theta}} (y|t,z)$ in place of $p_{\boldsymbol{\theta}} (Y^*\tighteq~y|T^{*}\tighteq~t,Z^*\tighteq~z)$. Hence, we can write our assumption as:
    \begin{equation}
        p_{\boldsymbol{\theta}} (y|t,z) = q_{\boldsymbol{\theta}} (y|t,z)\label{eq:y-given-zt-equal-in-two-settings}
    \end{equation}
    This notation should make it clear that whenever we switch $p$ to $q$ we are exploiting the assumption that this particular distribution function is the same in the interventional and the observed world.
    
    As specified by eq.~\ref{eq:y-given-zt-equal-in-two-settings}, the model parameters $\boldsymbol{\theta}$ are shared between the observed and the intervened-upon setting. We also further assume that all the observed examples $(Z_i, T_i, Y_i)$ and the intervened outcomes $(Z^*, T^*, Y^*)$ are independent given the model parameters $\boldsymbol{\theta}$. I.e. once we know the parameters, the duration of one person's headache, its severity and the dose they took is independent of how much aspirin someone else had taken, how long their headache lasted for, and its severity.
    
    Lastly, we can specify the distribution on the headache severity $Z^*$ in the intervened-upon setting. In this case, we can assume that we are interested in the effect in a person drawn from the same population as that in the observed data. Hence, we can specify that $Z^*$ is distributed in the same way as $Z$:
    \begin{equation}
        q_{\boldsymbol{\theta}}(z)=p_{\boldsymbol{\theta}}(z)
    \end{equation}
    
    In \Cref{fig:aspirin-example-interventions-twin}, a graphical model for the joint model over the two settings of interest is shown. The right-hand side corresponds to the hypothetical setting in which the system is subject to a manipulation on the dose-determining mechanism.
        
    \begin{minipage}{0.98\textwidth}
        \centering
        \vspace{0.4cm}
        \newlength{\tikzbayessep}
        \setlength{\tikzbayessep}{0.8cm}
        \centering
        \tikz[x=1.7cm,y=0.6cm]{

        \node[obs] (y) {$Y_i$};%
        \node[obs,above=of y, xshift=-1.5\tikzbayessep] (t) {$T_i$};
        \node[obs,above=of t, xshift=1.5\tikzbayessep] (z) {$Z_i$}; %
        \node[latent, above=of y, yshift=2.8\tikzbayessep, xshift=2.9\tikzbayessep] (theta) {$\boldsymbol{\theta}$}; 
        
        \node[obs, right=5\tikzbayessep of y] (ys) {$Y^*$};%
        \node[obs,above=of ys, xshift=1.5\tikzbayessep] (ts) {$T^*$};
        \node[obs,above=of ts, xshift=-1.5\tikzbayessep] (zs) {$Z^*$};
        
        % Text annotation of Interventional and observed world
        \node[fill=white, above of=z, node distance=1.2cm, inner sep=0pt,  xshift=-0.75\tikzbayessep] {\textsc{Observed world}};
        \node[fill=white, above of=zs, node distance=1.2cm, inner sep=0pt,  xshift=0.7\tikzbayessep] {\textsc{Intervened world}};

        \plate [inner sep=.35cm, yshift=0.01cm] {plate1} {(y)(t)(z)} {$i=1\dots N$}; %
        % edges
            \edge {theta} {z, t, y};
            \edge {theta} {ys, zs};
            \edge {z} {t, y};
            \edge{t} {y};
            \edge{zs} {ys};
            \edge{ts} {ys};
        }
        \centering
        \captionof{figure}{Graphical model for interventional inference in the aspirin example. The nodes $Z_i, T_i, Y_i$ on the left correspond to the cases in the observed world, whereas the nodes $Z^*, T^*, Y^*$ correspond to the hypothetical world in which we have intervened on $T^*$ --- it's no longer dependent on $Z^*$. Parameters $\boldsymbol{\theta}$ are shared between the two worlds allowing observations in the real world to inform inference in the intervened-upon one.
        \label{fig:aspirin-example-interventions-twin}}
        \vspace{0.4cm}
    \end{minipage}
     % From there on, the rules of probability prescribe how to combine the observations $\mathcal{D}$ to infer answers to questions in the interventional world.

    Based on the assumptions we have specified, we can write down a full joint distribution for the model:
    \begin{align}
        p(z^*&, t^*, y^*, \boldsymbol{\theta}, \mathcal{D}) =\\
        &= p(z^*, t^*, y^*| \boldsymbol{\theta}, \cancel{\mathcal{D}}) p(\mathcal{D}|\boldsymbol{\theta}) p(\boldsymbol{\theta}) \label{eq:joint-derivation-line-2}\\
        &= q_{\boldsymbol{\theta}}(z^*, t^*, y^*) \left(\prod_{i=1}^N p_{\boldsymbol{\theta}}(z_i, t_i, y_i) \right)p(\boldsymbol{\theta}) \\
        &= q_{\boldsymbol{\theta}}(z^*) q_{\boldsymbol{\theta}}(t^*|\cancel{z^*}) q_{\boldsymbol{\theta}}(y^*|z^*, t^*) \left(\prod_{i=1}^N p_{\boldsymbol{\theta}}(z_i) p_{\boldsymbol{\theta}}(t_i| z_i) p_{\boldsymbol{\theta}}(y_i | z_i, t_i) \right)p(\boldsymbol{\theta}) \label{eq:joint-derivation-line-4}\\
        &= \underbrace{p_{\boldsymbol{\theta}}(z^*) q_{\boldsymbol{\theta}}(t^*) p_{\boldsymbol{\theta}}(y^*|z^*, t^*)}_{\text{Interventional world}} \underbrace{\left(\prod_{i=1}^N p_{\boldsymbol{\theta}}(z_i) p_{\boldsymbol{\theta}}(t_i| z_i) p_{\boldsymbol{\theta}}(y_i | z_i, t_i) \right)}_{\text{Observed world}}p(\boldsymbol{\theta}) \label{eq:joint-derivation-line-5}
    \end{align}
    In eq.~\ref{eq:joint-derivation-line-2} we used the assumption that $(Z_i, T_i, Y_i)$ is independent of $(Z^*, T^*, Y^*)$ given $\boldsymbol{\theta}$, in eq.~\ref{eq:joint-derivation-line-4} the assumption that $T^*$ and $Z^*$ are independent, and in eq.~\ref{eq:joint-derivation-line-5} the assumptions $q_{\boldsymbol{\theta}}(z^*)=p_{\boldsymbol{\theta}}(z^*)$ and $q_{\boldsymbol{\theta}}(y^*|z^*, t^*)=p_{\boldsymbol{\theta}}(y^*|z^*, t^*)$.

    Given the joint, probability theory tells us how to find all the marginal distributions, conditional distributions and expectations of interest. How to actually compute the numerical values for these expressions (possibly approximately) then falls right within the realms of machine learning, statistics and deep learning.
    
    % Lastly, $p_{\boldsymbol{\theta}} (Y^*\teq y|T^*\teq t, Z^* \teq z) = p_{\boldsymbol{\theta}} (Y\teq y|T\teq t, Z \teq z)$ as mentioned previously. We could write a set of equations for this \textit{interventional} model in a corresponding way to eq.~\ref{aspirin-observed-model-eqs} for the observed model as follows:
    % \begin{equation}
    % \begin{aligned}
    %     Z^* &\sim \log\mathcal{N}\left(\mu_{Z}, \sigma_{Z}^{2}\right) && \\[5pt]
    %     T^* &= t^* \\
    %     Y^* &= \frac{(Z^*)^{b}}{(T^*)^c} \varepsilon^*_{Y} && \text {where  } \varepsilon^*_{Y} \sim \log \mathcal{N} \left(0, \sigma_{Y}^{2}\right) \\
    % \end{aligned}
    % \end{equation}
    % Where the parameters $\{b, c, \mu_Z, \sigma_Z, \sigma_Y\}$ are the same between the observed and interventional settings.

    \examplesec{Inference}
    Returning to the inference question, we wanted to know what's the expected headache duration in the intervened world in response to a given dose $t^*$. Hence, we can compute the expected value of $Y^*$ given the observed data $\mathcal{D}$:
    % Look into which equations need to be numbered
    \begin{align}
        \mathbb{E}[Y^*| \mathcal{D}] &= \int y^* p(y^*| \mathcal{D}) dy^* \label{eq:inter-integral-first}\\
        &= \int y^* p(y^*|t^*, \mathcal{D}) dy^* \hspace{5cm} \text{\small(using eq.~\ref{eq:intervention-marginal-is-cond})}\\
        &= \iiint y^* p(y^*, z^*, \boldsymbol{\theta} |t^*,  \mathcal{D}) dz^* dy^* d\boldsymbol{\theta} \\
        &= \iiint y^* p(y^*| z^*, t^*, \boldsymbol{\theta}, \cancel{\mathcal{D}})  p(z^*| \boldsymbol{\theta}, \cancel{t^*},  \cancel{\mathcal{D}})  p(\boldsymbol{\theta} |\cancel{t^*},  \mathcal{D}) dz^* dy^* d\boldsymbol{\theta} \label{eq:aspirin-internvetion-cancel}\\
        &=\iiint \underbrace{y^* q_{\boldsymbol{\theta}}(y^*| z^*, t^*)  q_{\boldsymbol{\theta}}(z^*) dz^* dy^*}_{\substack{\text{Calculate expectation in the intervened}\\ \text{world conditioned on posterior over }\boldsymbol{\theta}}} \underbrace{p(\boldsymbol{\theta} |\mathcal{D}) d\boldsymbol{\theta}}_{\substack{\text{Infer model parameters}\\ \text{using observed data } \mathcal{D}}}\label{eq:aspirin-interv-exp-in-terms-of-observed-dist}
    \end{align}
    
    where the cancellations in eq.~\ref{eq:aspirin-internvetion-cancel} follow from the conditional independencies in the model.
    
    Note that on line~\ref{eq:aspirin-interv-exp-in-terms-of-observed-dist}, all the distribution functions in the inner integral are the same as these in the observed distribution. For the log-normal aspirin model, we can actually calculate the inner expectation exactly:
    \begin{align}
        \iint y^* p_{\boldsymbol{\theta}}(y^*| z^*, t^*)  p_{\boldsymbol{\theta}}(z^*) dz^* dy^* = (t^*)^{-c}\exp{\left( b\mu_Z + \frac{b^2\sigma_Z^2+\sigma_Y^2}{2} \right)} \label{eq:aspirin-intervention-expectation-anal-formula}
    \end{align}% TODO: actually verify all of these, I'm fearing for my life I made a typo.
    As expected, the effect of assigning a different dose of aspirin $t^*$ is only determined by the parameter $c$; as long as $c>0$, intervening to administer a higher dose will in expectation shorten the headache duration.
    
    In this example, for an appropriate choice of a prior on $\boldsymbol{\theta}$, the integral in eq.~\ref{eq:aspirin-interv-exp-in-terms-of-observed-dist} could be calculated exactly, as the model is just a Linear Gaussian model in the log-space\footnote{Specifically, when $b, c$ are normally distributed, and $\sigma_Z, \sigma_Y$ follow an inverse-gamma distribution, $p(\boldsymbol{\theta})$ becomes a conjugate prior for this model.}. Alternatively, we could approximate $p(\boldsymbol{\theta}|\mathcal{D})$ with, for instance, the maximum-a-posteriori (MAP) estimate $p(\boldsymbol{\theta}|\mathcal{D}) \approx \delta(\boldsymbol{\theta} - \boldsymbol{\theta}_{\text{MAP}})$ or the maximum-likelihood estimate $p(\boldsymbol{\theta}|\mathcal{D}) \approx \delta(\boldsymbol{\theta} - \boldsymbol{\theta}_{\text{ML}})$, where $
        \boldsymbol{\theta}_{\text{ML}} = \argmax_{\boldsymbol{\theta}} p(\mathcal{D}|\boldsymbol{\theta})$.
    
    We can then consider the expected value of $Y^*$ under two different interventions $t^*=t^*_1$ and $t^*=t^*_2$. Using eq.~\ref{eq:aspirin-intervention-expectation-anal-formula}, we can calculate the effect of doubling the aspirin dose by setting $t^*_2 = 2 t^*_1$:
    \begin{equation}
        \frac{(t_2^*)^{-c}\exp{\left( b\mu_Z + \frac{b^2\sigma_Z^2+\sigma_Y^2}{2} \right)}}{(t_1^*)^{-c}\exp{\left( b\mu_Z + \frac{b^2\sigma_Z^2+\sigma_Y^2}{2} \right)}} = \left( \frac{t_2^*}{t_1^*} \right)^{-c} = \left( \frac{2 t_1^*}{t_1^*} \right)^{-c} = 2^{-c}
    \end{equation}
    Hence, according to the model, doubling the aspirin dose has the effect of reducing the headache duration by a factor of $2^{-c}$.
    % TODO: actually verify this??.
}

==> causal-discovery.tex <==
% So far, we have considered how to specify a joint model for the observed and intervened-upon settings to answer causal questions. The construction of this model requires the user to explicitly express their assumptions about how the settings are related. This is equivalently the case for Pearl's Causal Bayesian Networks - to construct one, you need domain-expertise to specify how the settings are related. Once these assumptions are laid out, we can make inferences about these novel settings. This is the essence of causal inference.

% Besides constructing a model to answer a question of a causal inference from data - causal inference - there is also the field of causal discovery.

% On the other hand, one could consider the problem of trying to infer how the intervened-upon setting and the observed setting are likely to be related solely from observed data. 

% It would be good to emphasise that our arguments mainly relate to causal inference.

% \todo{consider below point}
% In causal discovery, consider trying to infer the graph structure. If we were trying to infer the graph for a Bayesian Network, then which member of the Markov Equivalence Class is considered does not play a role. In other words, purely probabilistically, each member of the Markov Equivalence Class will be supported by the same \emph{evidence}. Given a uniform prior, the posterior probability of each member of a Markov Equivalence Class will be the same.

% On the other hand, consider a model classes in which the independence assumptions of the Bayesian Network are coupled with a prior on the form of the conditional probability along each directed edge, or assumptions on the form of that conditional probability. This assumption could be expresssed as the relationship having a functional form with an exogeneous noise variable (like in Structural Causal Models), and the assumptions could be placed on the functional form. Alternatively, a prior could be placed on the conditional probability according to its algorithmic complexity (see Scholkopf et al, Solomonoff General inductive inference). In these cases, we can distinguish between members of a Markov Equivalence Class, because the graph no longer only reflects the indepence assumptions. 




%What's the goal of causal discovery? It is to infer the "causal structure" of the variables. 

% The philosophy of causality and time?
But isn't the causal structure determined by time precedence? Namely, doesn't one variable have to necessarily preceed the other one in time to cause it?

Not necessarily, we could be dealing with aggregate data.

Consider for instance, trying to infer the price of which stocks causally affects which stocks. (in reality, the price of each stock likely affects all others at the next time step, but assume it's only a few). At each time step at the stock exchange, the current prices are sent out to traders, and the traders send in buy and sell orders which determine the prices at the next time step. Clearly, the value of each stock at time step $t+1$ is determined by the prices of a subset of stocks at time step $t$ (and possibly the time before that, but simplify with the Markov assumption). The mechanism determining the next value is the interaction of the traders with the stock exchange.

As we are amateurs, we do not get access to per time-step data, and only get aggregate statistics for each hour: i.e. the average price for each hour of trading. 

==> introduction_old.tex <==


\section{Introduction}

% The opening could certainly be stronger
In recent years, we have been struck by the fact that eminent researchers in the area of causality and statistical inference appear to hold contradictory views on the technical foundations of their field. The broader disagreement is well exemplified by the argument between Judea Pearl and Andrew Gelman; whereas Judea Pearl holds the position that \textit{``there is no way to answer causal questions without snapping out of statistical vocabulary''} \cite{quantainterviewpearl}, Andrew Gelman states that \textit{``I find it baffling that Pearl and his colleagues keep taking statistical problems and, to my mind, complicating them by wrapping them in a causal structure''} \cite{gelman2019statistical}.

\vspace{5pt}
\begin{displayquote}
    $\mathcal{Q}$: People are excited about the possibilities for AI. You’re not?
\\
\textit{``As much as I look into what’s being done with deep learning, I see they’re all stuck there on the level of associations. Curve fitting.''}
\\[-28pt]
\begin{flushright}  {{\rm --- Judea Pearl \cite{quantainterviewpearl}\hspace*{1.1cm}}} \end{flushright}
\end{displayquote}

The debate largely followed after the release of ``The Book of Why'' \cite{pearl2018book} and an interview with its author Judea Pearl \cite{quantainterviewpearl}, an excerpt of which is shown above. In the book, the author introduces causal thinking into statistics and machine learning. Simultaneously, he also presents a rather dim view on these fields. In a broad sweep Judea Pearl paints modern statistics, for example, as ``a model-blind data-reduction enterprise''. %Mention he wants people to use the do-calculus

% Both parties are highly esteemed academics on the topic of causality; Andrew Gelman is a Professor of statistics at the Columbia University and has authored many statistics books including chapters on causality. Judea Pearl is a Turing award winner who has written entire books on the topic. As such, it is particularly striking that they struggle to reach a consensus on the technical foundations of their fields.
Both parties are highly esteemed academics on the topic of causality; Andrew Gelman has authored many statistics books which cover the topic of causal inference. Judea Pearl is a Turing award winner who made many fundamental developments to the graphical approach to causality and has written multiple books on the topic. As such, it is particularly striking that they struggle to reach a consensus on the technical foundations of their fields.

These statements consequently propelled a larger discourse on the topic of causality and its relation to machine learning and statistics. The debate ranges across topics such as: do you need bespoke methods advocated by Pearl to do causal inference; how does previous work related to causality within machine learning and statistics fit in with Pearl's framework; and --- a question of a particularly semantic nature --- whether deep learning can perform causal inference.

% Mention semantical debate: can deep learning do causal inference?

% . The broader macro-level disagreement permeates down to the micro-level.
There is a lack of consensus about the micro-level technical details that echoes the landscape of the broader disagreement.
For instance, some contend whether graphical models alone can be used to answer certain types of causal questions -- e.g. counterfactuals.
In their book, Jonas Peters, Dominik Janzing and Bernhard Schölkopf write that \textit{“causal graphical models are not rich enough to predict counterfactuals”}.
Instead, they claim that a class of models called structural causal models (SCMs) is necessary:   \textit{``Formally, SCMs contain strictly more information than their corresponding graph and law (e.g., counterfactual statements)''} \cite{peters2017elements}. On the other hand, Kusner, Loftus and Russell et al., for instance, use causal graphical models to reason about questions of counterfactual nature in their paper on counterfactual fairness \cite{NIPS2017_6995}.


%Determining causal relationships from data is at the heart of statistics and much of modern science. It is for that reason striking that eminent statisticians seemingly hold contradictory views on the technical foundations of their field. What exactly lies at the roots of the disagreements?

% what is this paragraph saying?
% Lack of clear literature confuses novices
% We get to the bottom of claims by others using language of probabilistic modelling
% lack of clear examples -> we provide those

% lack of clear literature and examples. -> confusing to people new to ML
% We provide clear literature and examples
The lack of clear literature and a unified consensus in the field has induced confusion in those less familiar with the topic of causality. As an outsider to the field it's particularly hard to discern the meaning behind grand-sounding statements like "deep learning can't do causal inference". This confusion is further amplified by a seeming a lack of concrete examples illustrating how to utilise statistical methods to answer causal questions. We aim to address this short-coming, and clearly illustrate and explain how Pearl's causal framework relates to problems and methods encountered in machine learning. Specifically, our objective is to get to the bottom of various claims made by Judea Pearl and others using the language of probabilistic modelling and inference.

% In this note, we will approach causal inference from a probabilistic modelling perspective.  Concretely, we'll show how to model causal inference problems can be represented using a probabilistic modelling approach. Only then will we compare and contrast various approaches advocated for in the field of causality, and discuss various claims about their utility. 

Firstly, we aim to introduce the fundamental concepts and challenges relating to causal inference. In section~\ref{sec:key-concepts} we endeavour to show examples of what constitutes a causal problem, and clearly describe the obstacles and common pitfalls inherent to those problems. Rather than introducing various causal frameworks such as Potential Outcomes or Causal Graphical Models from the start, we first explain the intricacies of causal inference through a unifying and familiar toolset of probabilistic modelling. Readers familiar with causal inference may wish to skip this section with the exception of example~\ref{examplebox:aspirin-intro}, which introduces a concrete model we'll refer to extensively throughout. We'll then show concrete examples of causal questions such as \textit{interventions} (section~\ref{sec:interventions}) and \textit{counterfactuals} (section~\ref{sec:counterfactuals}), and in each case describe how one can approach tackling these within the probabilistic modelling framework.

Secondly, we'll address the claim that you \emph{need} a bespoke causal framework or notation to do causal inference. Pearl and others have alleged that without the \textit{do}-operator, attempting to answer causal questions is all but hopeless. In this note, we'll show that you \emph{can} in fact approach causal inference without resorting to these tools; the probabilistic modelling approach is sufficient.
We'll relate the probabilistic modelling approach introduced in sections~\ref{sec:interventions} and~\ref{sec:counterfactuals} to other causal inference frameworks. Namely, we'll introduce the methodology advocated in Pearl's ``The Book of Why'', including Causal Graphical Models (section~\ref{sec:pearls-single-model}) and Structural Causal Models (section~\ref{sec:scm}), and show how these can be made equivalent to the probabilistic modelling approach. We'll see under what conditions they are a special case of said approach. In the context of causal inference within the realm of machine learning, we'll discuss the nature and the proposed utility of the \textit{do}-notation, and demystify the purpose of the \textit{do}-calculus (section~\ref{sec:do-calculus}).

%  we will demonstrate how to answer causal questions of the kind of \textit{interventions} and \textit{counterfactuals} using probability theory and probabilistic modelling. In sections  will address how graphical models --- specifically, Bayesian Networks --- can be used for setting up models and specifying assumptions necessary to tackle problems of causal nature. We will illustrate this approach with concrete examples of causal inference problems, resolving the allegation that the standard probabilistic toolkit is not fit for answering causal questions.

Lastly, we'll demonstrate how deep learning tools can be used within a probabilistic modelling programme to tackle causal inference problems. We'll see concrete illustrative examples of inference problems on which methods from supervised and unsupervised learning --- such as deep neural networks and amortised variational inference --- can be applied.

% The reader should take away X
Hopefully, by the end of this note, the reader should come away with a clear understanding of how the methods from machine learning and statistics can be used to tackle causal problems, and a sense of appreciation for the challenges inherent in causal inference.

{\scshape \bfseries Prerequisites}
This note assumes familiarity with probabilistic machine learning and with the basics of graphical models; in particular, knowledge of Bayesian Networks --- on which much of Pearl's causal framework is based --- and \textit{d}-separation will be useful. For an introduction to graphical models and Bayesian Networks see e.g. \citep[\textsection8]{pearl2000causality,murphy2001introduction,bishop2006pattern}, or \Cref{appendix:bayesian-networks-def} for a summary.

==> markov-equivalence-old.tex <==

\subsection{Markov Equivalence Class}
We mentioned that there are caveats to defining a single Bayesian Network on the observed world, and the BN on the interventional world implicitly from it. Equivalence classes of BNs make doing so ambiguous.

Namely, there can be multiple different Bayesian Networks with different graphs that give the same set of conditional independencies, and hence entail the same factorisation of the joint distribution. They are said to belong to the same \textit{Markov Equivalence Class}. Recall that in the definition of a Bayesian Network, the graph was solely used to define said conditional independencies. Hence, all members of a Markov Equivalence Class imply the same restrictions on the joint distribution.

To give a concrete example of a Markov Equivalence Class, consider the graph in fig.~\ref{fig:aspirin-example} for the aspirin example. That graph does not entail any conditional independencies; the factorisation that we obtain from that Bayesian Network --- $p(y, t, z) = p(y| t, z) p(t|z) p(z)$ --- is valid for \textit{any} probability distribution by the product rule of probability functions. Hence, any rearrangement of the edges that results in a Directed Acyclic Graph, as shown in fig.~\ref{fig:aspirin-markov-eq}, yields the same set of conditional independencies. % TODO:{potentially include Markov Chain example}
\input{figures/markov-equivalence-classes.tex}

For the purposes of fitting the observed distribution only, it makes no difference which of the Bayesian Networks in the Markov equivalence class is being considered, as they all imply the same restrictions (in terms of conditional independencies) on the observed distribution. Hence, if we tried to infer the graph by estimating the conditional independencies from observed data, we could only distinguish between different Markov Equivalence Classes, but not between the members of each class. Even in the limit of infinite data ---  there is no statistical test on the observed data to uniquely determine a member from within the equivalence class. 

Despite the fact that the exact graph non-uniquely defines these independence assumptions, different graphs in the equivalence class can entail different interventional distributions through applications of the rule in def.~\ref{def:interventions}. Which graph from the Markov Equivalence Class the rule is being applied \emph{does} make a difference. For instance, an atomic intervention on $T$ in the 6th graph in \Cref*{fig:aspirin-markov-eq} would make $T^*$ independent of $Z^*$ and $Y^*$ in the intervened-upon setting, whereas same intervention on $T$ for the 3rd graph wouldn't introduce any independencies.

Hence, if we use a single BN on the observed variables and intend to use it for interventional inference, we have to be careful to select the right graph that will give us the interventional distribution that we desire.
In other words, when specifying a BN on the observed world in this way, we have to additionally make the assumption that for any intervention considered, applying the rule in def.~\ref{def:interventions} to the BN will yield the interventional distribution that we are interested in. We could fuse the definition of Bayesian Networks with this extra assumption to define a new model class --- a \emph{Causal Bayesian Network} \citet[p.~23]{pearl2000causality}.
By defining a Causal Bayesian Network, we are explicitly saying that for any intervention considered, applying the rule in definition~\ref{def:interventions} will yield the \emph{right} interventional distribution.

Although this corresponds to the definition given by Pearl in his book ``Causality''\citet[p.~23]{pearl2000causality}, it differs from the definitions given by other authors. For instance Sch\"olkopf, Janzing, and Peters define a Causal Graphical Model (their name for a Causal Bayesian Network) as a Bayesian Network in which each directed edge is assumed to correspond to a `causal' relationship \cite{peters2017elements}. However, as `causal' is an overloaded and ambiguous term, this definition somewhat obfuscates the true assumptions given above. Namely, that with a Causal Bayesian Network we are implicitly defining an interventional distribution for every intervention possible.\todo{see if footnote still needed}
\footnote{Pearl would motivate the definition of the term \textit{causal} by saying that one variable causally affects the other when an intervention on that variable would change the distribution on the other variable. This interpretation of the word causal is later used to define a Causal Bayesian Network/Causal Graphical Model by some authors, and to state that in a Causal Bayesian Network the rule in def.~\ref{def:interventions} will give the desired interventional distribution.
This partly circular definition obfuscates where and in what form subjective expert opinion comes in to define these assumptions.
}

It is easy to get confused by the different definitions -- which part are a mathematical construct, and at which part are we making assumptions by linking these constructs to real-world objects.
It's not hard to imagine that this is confusing to many.
This has pushed some to humorously defining Causal Bayesian Networks as Bayesian Networks with the word `causal' prepended to them \citep{TacoCohenTalkCausalModelAbstraction2022}.

% Interventions (as defined above) are nothing but operations on graphical models and subsequent probabilistic inference. The causal interpretation of the results, however, depends on the assumption about the desired meaning of what the edges represent and what removing them entails. By specifying a joint model over all the settings of interest, such as the joint graphical model in fig.~\ref{fig:aspirin-example-interventions-twin}, we are explicitly making such assumptions.

% This is even further complicated when we consider that there might be unobserved latent variables. This motivates the field of causal discovery...  what assumptions are necessary to identify the most probable... (Maybe mention model evidence? Bayesian model selection).

% \todo{maaaybe reintroduce the mnist example}

% To give a concrete example of the kind of choices a practitioner has to make at model specification time
% Consider, for instance, an MNIST example where the dataset consists of images $\mathbf{x}$ and digit labels $y$. Do the images cause the labels, or do the labels cause the images? It's a somewhat silly question that we don't have to bother answering when we specify a joint model over the observed data and the interventions of interest. For instance, if the interventional question is - what if I were to show a human labeler a picture from an augmented distribution on $\mathbf{x}$ - it is immediately obvious how to specify a joint graphical model for this setting. Similarly, we could ask about the distribution over the images if we were to alter the distribution over digits given to a hypothetical scribe. One could say that in one scenario the digits cause the images, and in other the images cause the digits; by specifying a joint model for the interventional and the observed setting we are explicitly making modelling assumptions that one could choose to call \emph{causal}.

Note that this is a complete non-issue when using a joint model over all the settings of interest. By specifying a complete joint model over all the relevant tasks --- like we did in the aspirin example --- we are forced to explicitly make the assumptions about how these tasks are related. Hence, you can either choose to specify a single model over the observed setting while being mindful of the implicit assumptions and the Markov Equivalence Classes, or you can specify a joint model where the assumptions are crystal clear.


==> old-figures-and-text.tex <==

% \begin{figure}
% \newlength{\tikzbayessep}
% \setlength{\tikzbayessep}{0.8cm}
% \centering
%   \tikz[x=1.7cm,y=0.6cm]{

% % nodes
% %  \node[obs] (x1) {$X_1$};%
%  \node[obs] (y) {$Y$};%
%  \node[obs,above=of y, xshift=-1.5\tikzbayessep] (t) {$T$};
%  \node[obs,above=of t, xshift=1.5\tikzbayessep] (z) {$Z$}; %
%  \node[latent, above=of z,xshift=2.5\tikzbayessep] (theta) {$\mathbf{\theta}$}; 
 
%  \node[obs, right=5\tikzbayessep of y] (x1s) {$Y^*$};%
%  \node[obs,above=of x1s, xshift=-2\tikzbayessep] (x2s) {$X_2^*$};
%  \node[obs,above=of x1s] (x3s) {$X_3^*$}; %
%  \node[obs,above=of x3s,xshift=-0.84\tikzbayessep] (x4s) {$X_4^*$}; %

%  \plate [inner sep=.25cm,yshift=.2cm] {plate1} {(x1)(x2)(x3)(x4)} {$N$}; %
% % edges
%     \edge {theta} {x1s, x2s,x4s};

%     \edge {x2s} {x4s};
%     \edge{x3s} {x4s}; % edges from theta to x1?
%     \edge{x1s} {x2s}
%   }
%  \caption{Example graphical model for interventional inference. The nodes $X_1, \ldots, X_4$ on the left correspond to the observed examples in the observed world. Those examples can be used to estimate the parameters $\boldsymbol{\theta}$ of the conditional distributions. The nodes $X_1^*, \ldots, X_4^*$ correspond to the hypothetical world in which we've intervened on $X_3^*$ (in this case, we've given it an empty set of parents). This world shares the remaining conditionals $p_\theta (x_i^*|x_{\mathbf{PA*}_{i}})$ with the observed world, and hence shares the learnt parameters $\boldsymbol{\theta}$}
%  \label{fig:graphical-model-interventional-inference1}
% \end{figure}


% TODO: consider where to put this
% Much of the confusion around causality stems from the choice of the right modelling tool; namely, whether to use \emph{Causal Graphical Models} or \emph{Structural Causal Models}, both of which are described in Judea Pearl's book \textit{``Causality''} \cite{pearl2000causality}. Here we'll aim to introduce the two approaches. First, we'll start with a definition of Bayesian Networks which underlie both approaches:

% This additional interpretation of edges as corresponding to causal mechanisms is necessary for causal inference. It allows for the results of manipulation on that graph by removing or replacing edges (and the conditional probability functions associated with them) to be interpreted as some physically plausible alteration to the generative process. This will become more apparent after introducing interventions in the section below.

\begin{itemize}
    \item In aspirin example in eq. we obtained an expression for the conditional in the interventional part of the model in terms of conditional density functions from the observed world - i.e. those that were shared between the two.
    \item specifically, conditioning on variable $z$ allowed us to do so. This is called ``adjusting'' for $Z$.
    \item How to express the conditional of interest in the intervened-upon world in terms of conditionals from the observed world and $g^*$ in a more complex case?
    \item Consider the brute force solution. In general, as def.~\ref{def:interventions} gives a definition for the joint, we can obtain any desired conditional distribution of interest by marginalising out. Leads to potentially very big integral. And what if the integral has unobserved variables? Can we do better?
    \item In the case of an atomic intervention on $x$, adjusting using the parents of $x$ is sufficient. Potentially much simpler than previous expression.
    \item Pearl proposes other such ``adjustments'' (backdoor criterion and toward necessity)
    \item What happens when some variables are unobserved, and hence we might not be able to directly estimate conditionals with them? 
    \item Pearl has developed a so-called \textit{do}-calculus. We will not give its rules here, they can be found in \citet[Section~3.4]{pearl2000causality} (maybe put in appendix as well to satisfy curiosity if someone is reading the doc). The \textit{do-}calculus allows for finding expressions for all identifiable intervention distributions with a repeated application of its rules (which you'd hope seeing as you can do this by using definitions~\ref{def:bayes-net} and~\ref{def:interventions} and the rules of probability theory). Using the \textit{do}-calculus Tian [2002] has developed an algorithm that is guaranteed to find all identifiable intervention distirbutions, and Schipster and Pearl have developed a graphical criterion on $\mathcal{G}$ for determining identifiability of an interventional distribution.
    \item The \textit{do}-calculus simply builds on the rules of probability theory, the definition of a BN and the definition of interventions in BNs. The choice to include `calculus' in its name adds a ring of profoundness to it and inspires curiosity, instilling a somewhat distorted expectation of what it actually is.
\end{itemize}

==> potential-outcomes.tex <==
\subsection{Potential Outcomes}\label{sec:potential-outcomes}
An alternative framework for causal inference that has gathered much renown is the Potential Outcomes framework. We'll briefly introduce it from the perspective of probabilistc modelling, to illustrate how all the frameworks link together.

% TODO: this might not be necessary
Returning to the aspirin problem, let's temporarily constrain ourselves to a simpler problem, one in which we consider only two treatments: a big dose and a small dose.

% Consider Y_i,t < it's a random variable.
Returning to the aspirin problem: for each example $\{Z_i, T_i, Y_i\}$, we can consider counterfactual random variables $Y_i $


% Our clearly defines a joint distribution on those Y_i, ts

% Potential outcomes framework would take these potential outcomes as primitives.


% We can consider the effect of 


It should be clear that we do not necessarily \emph{need} to use a Bayesian Network (or any extensions thereof such as Structural Causal Models or Causal Graphical Models) to do causal inference. Consider, for instance, marginalising out the variable $Z$ from the model in X. We got the following expression for the joint distribution over the remaining variables:

% The set of conditional independecies in this All we need to do is to specify a model of how the two settings are related. To   This might appear as a slightly obvious point

We might prefer the original formulation (graphical model plus form of conditionals) when describing a model, as the assumptions are more interpretable in that form.

==> predator-prey-example.tex <==
\examplebox{Predator-prey counterfactuals}{
\examplesec{Inference problem}
Imagine that fishermen in some region of the world decided to cull their local seal population, driven by anecdotal fears about the danger to the fish population on which the fishermen rely. Some months later, that seal becomes an endangered species. There has since been a court case looking into the culling practices and the jury is wondering if the fishermen are responsible for the species' endangerment. They want to know: in retrospective, what would the seal population have been had it not been culled earlier?

To concretely formulate the counterfactual problem: we have observations of the immediate pre-cull, post-cull and current seal populations. These are denoted $s_1^*$, $s_1$ and $s_2$ respectively. We do not, however, have observations of either the initial, or the final fish populations in your region, as there are plenty of fish in the sea. The initial fish population is a latent, unobserved variable. From these observations, and the available data on fish and seal population elsewhere, we want to answer as accurately as possible what the seal population would have been now, had it been kept at the pre-cull level earlier. The task is illustrated in figure \ref{fig:inference-task-illustration}.

% FIG: Illustration of causal inference problem
\begin{minipage}{0.99\textwidth}
    \vspace{0.3cm}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/counterfactual-inference-sealfish-illustrative.eps}
    \captionof{figure}{Illustration of the causal inference problem.\label{fig:inference-task-illustration}}
    \vspace{0.3cm}
\end{minipage}

\examplesec{Data}
The data in this example is based on a dynamics model of predator and prey populations. Specifically, the populations' evolution over time is simulated with the Lotka-Volterra differential equations (also known as the predator-prey equations):
\begin{align}
\frac{d f}{d t} =\gamma_1 f-\gamma_2 f s &&
\frac{d s}{d t} =\gamma_3 f s-\gamma_4 s \label{eq:lotka-volterra}
\end{align}
Here, $s$ represents the seal (predator) population and $f$ represents the fish (prey) population.  $\gamma_1, \gamma_2, \gamma_3, \gamma_4  \in \mathbb{R}_{>0}$ are the parameters of the equations that determine the population dynamics. Examples of population oscillations generated from these equations are shown in figure \ref{fig:example-dynamics-lotka-volterra}. % explaining the symbols.

\begin{minipage}{0.98\textwidth}
    \vspace{0.5cm}
    \centering
    \includegraphics[width=0.87\textwidth]{figures/example_lotka_volterra_dynamics.eps}
    \captionof{figure}{Example population oscillations generated by the Lotka-Volterra equations.}
    \label{fig:example-dynamics-lotka-volterra}
    \vspace{0.6cm}
\end{minipage}
}{examplebox:predator-prey}

In a practical scenario, a practitioner would not have access to the simulator itself, but rather only to some data generated from it. As such such, they would have to resolve to using statistical techniques to estimate the population dynamics. For this example we assume that the fish and seal population dynamics are dictated by the pair of equations~\ref{eq:lotka-volterra} with a fixed set of parameters $\gamma_1\teq0.015, \gamma_2\teq0.012, \gamma_3\teq0.007, \gamma_4\teq0.009$. The dataset available consists of tuples $\mathcal{D}=\{( f_{1,i}, s_{1,i}, \tau_i, f_{2, i}, s_{2,i} )\}_{i=1}^N$ where $f_{1,i}, s_{1,i}$ are the initial fish and seal populations, and $f_{2, i}, s_{2,i}$ are the populations after time $\tau_i$. A model can then be fitted to this data to predict the seal and fish population after some time $\tau$ given the initial fish and seal populations: $p_\theta (s_2, f_2 | s_1, f_1, \tau)$. For simplicity, we'll assume a fixed $\tau\teq 400$.
% The simulator allows us to construct a simple counterfactual inference problem to benchmark various inference approaches. Specifically, we can ask what the fish and seal populations would have been after some time, had the initial conditions been different. As we have access to the underlying simulator, any counterfactual query can always be computed exactly and compared against. The problem is conceptually simple, but can be made non-trivial if the initial conditions are only partially observed. Furthermore, the relationship between populations at different times is highly non-linear. This necessitates the use of more expressive machine-learning methods such as neural networks or Gaussian processes.

\exampleboxcont{
\examplesec{Model and assumptions}
We can again represent our assumptions by setting up a joint model over the variables in the observed world $S_1$, $S_2$ and $F_1$ (where $F_1$ is unobserved), and the corresponding variables in the counterfactual world $S_1^*$ and $S_2^*$. We assume that the initial fish population $F_1$ is the same in both the counterfactual and the observed setting. We can then specify further assumptions about the problem with a graphical model over all the settings of interest, as shown in \Cref{fig:seal-fish-twin-network1}.


% FIG: Graphical Model
\begin{minipage}{0.99\textwidth}
\centering
  \tikz{
% nodes
 \node[obs] (s2) {$S_2$};%
 \node[obs, right=4.2cm of s2] (s2star) {$S_2^*$};%

 \node[obs,above=of s2,xshift=-0cm,fill] (s1) {$S_1$}; %
 \node[latent,above=of s2,xshift=2.4cm] (f1) {$F_1$}; %
 \node[obs,above=of s2star,xshift=0cm,fill] (s1star) {$S_1^*$}; %
 \node[latent,above=of f1, yshift=-0.6cm] (theta) {$\boldsymbol{\theta}$};
    % Text annotation of counterfactual and observed world
    \node[below of=s2, node distance=0.8cm, inner sep=0pt,  xshift=0.0\tikzbayessep] {\textsc{Observed world}};
    \node[below of=s2star, node distance=0.8cm, inner sep=0pt,  xshift=0.0\tikzbayessep] {\textsc{Counterfactual world}};

% edges
 \edge {s1,f1} {s2};
  \edge {s1star,f1} {s2star};
  \edge {theta} {s2star, s2} }
 \captionof{figure}{Graphical model corresponding to the inference problem. The dependence of the fully observed dataset $\mathcal{D}$ on $\boldsymbol{\theta}$ has been omitted for conciseness.\label{fig:seal-fish-twin-network1}}
 \vspace{0.2cm}
\end{minipage}

From there on, the joint distribution over all the variables follows:
\begin{align}
    &\ p(s_1, s_2, f_1, s_1^*, s_2^*, \mathcal{D}) = 
    p(s_1, s_2, f_1, s_1^*, s_2^* | \boldsymbol{\theta}, \cancel{\mathcal{D}}) p(\mathcal{D}|\boldsymbol{\theta}) p(\boldsymbol{\theta}) \label{eq:counterfactual-pred-prey-joint-line-1} \nonumber \\
    &= \Big( p(f_1|\cancel{\boldsymbol{\theta}})p(s_1|\cancel{f_1}, \boldsymbol{\theta})p(s_2|s_1, f_1, \boldsymbol{\theta}) p(s_1^*|\cancel{s_2}, \cancel{s_1}, \cancel{f_1}, \cancel{\boldsymbol{\theta}}) p(s_2^*| s_1^*, \cancel{s_2}, \cancel{s_1}, f_1, \boldsymbol{\theta}) \Big)  p(\mathcal{D}|\boldsymbol{\theta}) p(\boldsymbol{\theta}) \nonumber \\ % \label{eq:counterfactual-pred-prey-joint-line-2}  \\
    &= \Big( \underbrace{p(s_1) p_{\boldsymbol{\theta}}(s_2|s_1, f_1)}_{\text{Observed world}} \underbrace{p(f_1)}_{\substack{\text{Shared}\\ \text{in both}}} \underbrace{q(s_1^*) q_{\boldsymbol{\theta}}(s_2^*| s_1^*, f_1)}_{\text{Counterfactual world}} \Big)  p(\mathcal{D}|\boldsymbol{\theta}) p(\boldsymbol{\theta}) % \label{eq:counterfactual-pred-prey-joint-line-4}
\end{align}
In the derivation, we again exploited the conditional independencies in the graphical model. We can further assume that the mechanism determining the final seal population with the observed world is the same as that in the counterfactual, i.e. $q_{\boldsymbol{\theta}}(s_2| s_1, f_1)=p_{\boldsymbol{\theta}}(s_2| s_1, f_1)$. 

We further assume that we know $S_1\sim \log \mathcal{N}(0, 1)$ and $F_1\sim \log \mathcal{N}(0, 1)$. 
}
Hence, the only distribution we need to learn the parameters for is $p_{\boldsymbol{\theta}}(s_2| s_1, f_1)$. As the distribution on $S_2$ conditioned on $S_1, S_2$ is highly nonlinear, we can choose to represent it with a deep neural network. Specifically, we will use a neural network that parameterises a Gaussian distribution: $p_{{\boldsymbol{\theta}}}(s_2| s_1, f_1)=\mathcal{N}(s_2;f_\theta(s_1, f_1), \sigma^2)$ where the mean $f_\theta(s_1, f_1)$ is modelled with a neural network, and the standard deviation $\sigma=10^{-2}$ is fixed.

We could set the the distribution $q(s_1^*)$ to a delta function as we did before; however, recall that setting $S_1^*$ to be delta-distributed and marginalising over it is equivalent to conditioning on $S_1^*\teq s_1^*$, as we saw in eq.~\ref{eq:intervention-marginal-is-cond}. Hence, we'll leave the distribution on $S_1^*$ unspecified and just condition on $S_1^*\teq s_1^*$ instead.

% Altogether, the counterfactual world is modelled as being identical to the observed world, except for the initial seal population. 

% In the counterfactual world, we wish to set the initial seal population $S_1^*$ to a different value than $S_1$ - the pre-cull seal population. We can then execute inference to predict the posterior over the final seal population in the hypothetical counterfactual world.

\exampleboxcont{
\examplesec{Inference}
Our inference objective was to compute the probability distribution over the current counterfactual seal population $S_2^*$, given that we observed the true initial seal population $s_1$, the true final seal population $s_2$, and in the counterfactual world the initial seal population is set to the pre-cull level $S_1^*\teq s_1$. To again mathematise the problem: we want to compute the probability distribution $p(s_2^*|s_1, s_2, s_1^*, \mathcal{D})$. This particular graphical model structure allows for the decomposition:
\begin{align}
    p(s_2^*|&s_1, s_2, s_1^*, \mathcal{D}) = \iint p(s_2^*, f_1, \boldsymbol{\theta}|s_1, s_2, s_1^*, \mathcal{D}) df_1  d\boldsymbol{\theta}\nonumber \\
    &=\iint p(s_2^*|s_1, s_2, \cancel{s_1^*}, \boldsymbol{\theta}, \cancel{\mathcal{D}}) p(f_1| \boldsymbol{\theta}, s_1, s_2, \cancel{s_1^*}, \boldsymbol{\theta}, \cancel{\mathcal{D}})  p(\boldsymbol{\theta}|s_1, s_2, \cancel{s_1^*}, \mathcal{D}) df_1 d\boldsymbol{\theta}\nonumber \\
    &= \mathbb{E}_{p({\boldsymbol{\theta}}|\mathcal{D}, s_1, s_2)} \Big[ \int p_{\boldsymbol{\theta}}(s_2^*|s_1^*, f_1)p(f_1|s_1, s_2, {\boldsymbol{\theta}}) df_1 \Big]\label{eq:exact-inference-objective-prey-predator-exp}
\end{align}
where:
\begin{equation}
 p(f_1|s_1, s_2, {\boldsymbol{\theta}}) \propto p_{{\boldsymbol{\theta}}}(s_2| s_1, f_1)p(f_1) \label{eq:posterior-over-fish1}
\end{equation}
We can put this back into eq.~\ref{eq:exact-inference-objective-prey-predator-exp} to obtain the following expression for the quantity of interest:
\begin{equation}
    p(s_2^*|s_1, s_2, s_1^*, \mathcal{D}) \propto \mathbb{E}_{p(\boldsymbol{\theta}|\mathcal{D}, s_1, s_2)} \Big[ \mathbb{E}_{p(f_1)} [ p_{\boldsymbol{\theta}}(s_2^*|s_1^*, f_1)p_{\boldsymbol{\theta}}(s_2|s_1, f_1) ] \Big] \label{eq:estimable-counterfactual-pdf-pred-prey}
\end{equation}
}

The above expression gives us a way to estimate $p(s_2^*|s_1, s_2, s_1^*, \mathcal{D})$. Firstly, the outer expectation over ${\boldsymbol{\theta}}\sim p({\boldsymbol{\theta}}|\mathcal{D}, s_1, s_2)$ can be approximated with a point estimate ${\boldsymbol{\theta}}_{ML}$ by likelihood maximisation on the dataset $\mathcal{D}$. In principle, the posterior takes the form $p(\boldsymbol{\theta}|\mathcal{D}, s_1, s_2)$, but we can assume that the influence of the additional sample $(s_1, s_2)$ is negligible, and take the maximum likelihood estimate w.r.t. just $\mathcal{D}$ instead. The inner expectation can be estimated by standard Monte-Carlo sampling. Thanks to $s_2^*$ being one-dimensional, this simple sampling procedure will suffice.

\begin{minipage}{0.99\linewidth}
    \centering
    \definecolor{lightblue}{RGB}{0,162,255}
    \definecolor{lightgreen}{RGB}{29,177,0}
    \includegraphics[width=0.9\textwidth]{figures/observed-and-all-posteriors-and-ground-truth.eps}
    \captionof{figure}{\textbf{\textcolor{lightblue}{Left:}} the inferred distribution over the initial fish population. \textbf{\textcolor{lightgreen}{Right:}} the counterfactual seal population had the initial fish population been kept at a pre-cull level. \textbf{Centre:} the actual simulated seal population dynamics for both the actual and the counterfactual initial conditions.\label{fig:inferred-posteriors-in-counterfactual-pred-prey}}
\end{minipage}

The outcome of this inference procedure for particular values of $f_1, s_1, s_2, s_1^*$ is shown in \Cref{fig:inferred-posteriors-in-counterfactual-pred-prey}. As can be seen, the posterior distribution over $F_1$ is bimodal, indicating that two different initial fish populations could have explained the observed example well. Consequently, the posterior over the counterfactual seal population $S_2^*$ is also bimodal. In either case, we can conclude from our model that had the fishermen not culled the seal population, in all likelihood the seal population would have been lower at the present date.%\footnote{This the case in our model, because the cull stabilised the oscillation of the fish and seal population dynamics}

% Is there a different way to approach this problem? A non-causal, more model-blind alternative would be, for instance, modelling the conditional distribution over the final seal population given the initial seal population - $p(s_2 | s_1)$ - while completely ignoring the fish population\footnote{In this method, for the prediction to have a causal interpretation (as what Pearl would describe as an intervention), an assumption that the initial seal population 'causes' the final seal population is still necessary.}. This distribution could again be approximated using the collected dataset $\mathcal{D}$. However, as the final seal population largely depends on the initial fish population, ignoring the latent variable yields a rather uninformative posterior.



==> some-other-points.tex <==

It is also important to consider the target audience of many of Pearl's remarks. For instance, in many science disciplines, controlling for as much as possible --- i.e. treating everything as a potential confounder --- is the ruling paradigm. Judea Pearl has, through his use of graphical models to represent the generative process, illustrated that controlling for all the variables is often unnecessary (increasing the uncertainty of the estimate), and in many cases inadequate.

When doing counterfactual inference, we assume that there are some unobserved set of latent variables $\mathbf{U}$ that capture some unobserved characteristics particular to the specific example/case at hand. 

In general, the probability of a counterfactual can be computed in three steps:
\begin{enumerate}
    \item \textit{(abduction)} Compute the probability distribution over the shared unobserved variables $\mathbf{U}$ given the observation: $p(\mathbf{U}=\mathbf{u}|\mathbf{X}=\mathbf{x})$
    \item \textit{(action)} Choose the (counterfactual) distribution of intervened upon variables in the counterfactual part of the model.
    \item \textit{(prediction)} Run inference in the counterfactual part of the model to obtain a counterfactual distribution over variables of interest.
\end{enumerate}
% Come up with a good example here where the counterfactual distribution might depend on the structural causal model, and both are a valid interpretation.

\examplebox{Skill rating and causal questions about games}{
    To give an idea of what sort of questions could be approached by the analysis, we'll consider predicting the outcomes of two-player games. We'll adopt a simplified two-player version of TrueSkill.
    
}

% Stability
As an aside, it is also often assumed that the causal graphical model satisfies \emph{stability}. This means that if the CGM is parametrised by parameters $\boldsymbol{\theta}$, there is no other parametrisation $\boldsymbol{\theta^*}$ that would remove any independencies in the distribution. I.e. there is no independence in the observed distribution purely due a specific choice of parameters that cancels out the dependence. This becomes less of an issue when we consider a distribution over $\boldsymbol{\theta}$ as in Bayesian approaches.

\todo[inline] {maybe, somewhere: Section on identifiability/ Connect to multiview models. (viewing faces from different directions).}

comment on mixture model version [can represent intervention by a mixture model instead]

Bayesian approach (set up to echo the structure of a counterfactual)

effects of causes [cite Pearl’s ‘twin’ setup which mirrors our own]

different versions of the probabilistic model

marginalise out the shared randomness, comment how this is not an SEM
correlated, rather than perfectly shared version and then the view that some randomness should be shared and some should be drawn anew from the prior

\todo{Add something about faithfulness}

causes of effects

talk about the setup as a shared model can lead to uncomfortable situation whereby we’d change our estimate of the noise that existed in the real world (and counterfactual) when we see data in the counterfactual world (this seems weird)
different view when posterior for real world forms prior for counterfactual world 

but, wrt predictions in the counterfactual world this results in the same computation as before by Bayesian updating, as long as we only consider variables in the counterfactual world. 

elements of causal reasoning in machine learning 

Pearl's argument in Causality chapter 2 on how fit to data is everything in machine-learning. Relate to meta-learning -> It is certainly advantageous in meta-learning approaches for the algorithm to 'learn' the causal structure.

Bayesian model based RL as a Bayesian intervention / counterfactual 

Bayesian active learning by disagreement — seems very like a causes of effects setup (given what I’ve currently seen, if I observed an output $y^*$ at $x^*$, what would my belief over the function look like)

David Sontag’s work

Mention Causal Bootstrap as an example of poor understanding.

Mention that there is something between counterfactuals (and nothing), namely, inferring over latent variables, but not over the noise.

multi-task models, multi-view models, inter-battery factor analysis as utilising the basic graphical modelling structure

Judea Pearl - Causality book review: (highly cited) http://bayes.cs.ucla.edu/BOOK-2K/neuberg-review.pdf

Close to our view-point
David Blei's work - 
Variational Fair Autoencoder - C louizos.
Counterfactual Fairness

==> technical-abstract.tex <==
\maketitle
% Motivation -> heated debates, many question whether you can do causal inference with ML
% Incorporate questions raised: can you do causal inference with machine learning? Do you need a special framework or notation to do causal inference?

